Counterfactual Fairness Is Basically Demographic Parity

Making fair decisions is crucial to ethically implementing machine learning algorithms in social settings. In this work, we consider the celebrated definition of counterfactual fairness [Kusner et al., NeurIPS, 2017]. We begin by showing that an algorithm which satisfies counterfactual fairness also satisfies demographic parity, a far simpler fairness constraint. Similarly, we show that all algorithms satisfying demographic parity can be trivially modified to satisfy counterfactual fairness. Together, our results indicate that counterfactual fairness is basically equivalent to demographic parity, which has important implications for the growing body of work on counterfactual fairness. We then validate our theoretical findings empirically, analyzing three existing algorithms for counterfactual fairness against three simple benchmarks. We find that two simple benchmark algorithms outperform all three existing algorithms -- in terms of fairness, accuracy, and efficiency -- on several data sets. Our analysis leads us to formalize a concrete fairness goal: to preserve the order of individuals within protected groups. We believe transparency around the ordering of individuals within protected groups makes fair algorithms more trustworthy. By design, the two simple benchmark algorithms satisfy this goal while the existing algorithms for counterfactual fairness do not.

==> Simplifying Counterfactual Fairness (AAAI)/backup.tex <==

%We present diagrams of these causal models in
%\ref{fig:morecausalmodels}.
%We ran the same experiments as we did for the law school data on the additional 
%datasets and found similar results.
%The figures for the additional experiments
%appear in Appendix \ref{sec:experiments}, as well as a link to our \href{https://anonymous.4open.science/r/simplifying_counterfactual_fairness-413B/}{\textbf{code}}, for reproducibility.
%
%Table \ref{tab:rmse} summarizes the error for each algorithm and
%example we consider.
%Of course, the full linear model (no fairness constraints)
%reliably achieves the lowest rMSE while Level 1 and Level 3 are close
%behind, since their predictions do not satisfy demographic parity.
%Level 2 tends to satisfy demographic parity but has higher error than
%Listing 1 and Listing 2.



%\subparagraph*{Experiments}
%Table \ref{tab:rmse} shows the rMSE for the six algorithms on
%all three data sets we explore: law school, default risk, and healthcare. As we discussed previously, we used the law school success data set from \cite{kusner2017counterfactual}.
%We sought a new real world data set that was not used in
%\cite{kusner2017counterfactual}:
%default risk is based on the Home Credit Default Risk data set \cite{kaggle}.
%We estimated a causal model based on observations of the default risk data, to mimic the ``domain expert'' process.
%We also sought to create a challenging synthetic data set that we could make match the causal model of a fake world almost exactly (because we could draw synthetic data directly from the fake structural model).
%Our synthetic data set on healthcare is very loosely based on \cite{obermeyer2019dissecting}. The synthetic scenario represents the ``ideal'' circumstance for counterfactual methods proposed by \cite{kusner2017counterfactual} where observations are
%drawn from the causal model.
%We include the figures for the structural causal models
%and prediction distributions in Appendix \ref{sec:experiments}.
%
%Our experiments with default risk demonstrated the difficulty in estimating a causal model (the ``domain expert'' process), and we noted that the ``levels'' proposed by \cite{kusner2017counterfactual} suffered from similar pitfalls to the law school example. For healthcare, because we had direct access to the ground truth causal model, Level 3 (which makes the strongest assumptions) performed well.
%However, direct access to a ground truth causal model is unrealistic. Across all the tests we conducted, our approaches (presented in Listings \ref{alg:normal} and \ref{alg:quantile}) consistently performed well while guaranteeing demographic parity and enforcing Assumption~\ref{req:preserve}.
% \vspace{-0.25cm}

%To derive the two simple algorithms for demographic parity,
%we used a strong assumption on the relative ranking of individuals
%made by a fair algorithm.
%Proposition \ref{prop:counterexample} shows that this assumption
%is not always true for counterfactually fair algorithms.
%We acknowledge that Assumption~\ref{req:preserve} may prevent us
%from producing the fairest model, from a causal perspective.
%However, we believe that preserved orderings are preferable to the
%highly unstable orderings in the levels of 
%\cite{kusner2017counterfactual}.
%One reason to prefer preserved orderings is that 
%even soft guarantees for relative orderings of within-group individuals 
%would lead to more transparent, trustworthy and ultimately 
%\textit{useful} counterfactually fair algorithms.
%Prior work already expands counterfactual fairness to deal with 
%between-group ranking \cite{yang2020causal}, and we hope that 
%our results encourage others to investigate counterfactually 
%fair models with theoretical guarantees.
%
%Under common distributional assumptions, we showed
%that counterfactual fairness implies demographic parity.
%This result offers a method for testing whether an
%algorithm is counterfactually fair.
%Furthermore, we derived two algorithms that satisfy demographic parity and
%preserve the ordering of outcomes within groups.
%Preserving the order of predictions within each
%group is a natural choice,
%we argue, when a causal model is unavailable.
%However, we show an example where a counterfactually fair
%algorithm induces a change in relative order.
%Our experiments on the three levels of counterfactual fairness proposed
%in \cite{kusner2017counterfactual} show that two of the
%three levels do not necessarily achieve demographic parity.
%Assuming the data is drawn from a distribution of latent variables
%that is independent of protected attributes, these findings
%suggest the two levels are not counterfactually fair.
%We further investigate the individual choices made by
%the levels and observe that individual predictions
%are highly unstable between different levels.
%We posit that even though preserving the order of predictions
%within groups is not always counterfactually fair,
%it is preferable to have a transparent and consistent
%policy over the apparent randomness in the three levels.
%
%We designed two algorithms to achieve demographic parity,
%which is a necessary condition for counterfactual fairness.
%% but they are not counterfactually fair.
%One important open question is how to design algorithms 
%with theoretical counterfactual fairness guarantees.

%In contrast, our two algorithms do preserve orderings
%in a principled manner while guaranteeing demographic parity.
%We believe that considering principled methods for automated 
%decision making procedures that account for protected
%attributes like race, gender, and age is vital for ethical
%implementations of machine learning,
%and leave open the problem of designing additional algorithms
%with counterfactual fairness guarantees.

==> backup.tex <==

%We present diagrams of these causal models in
%\ref{fig:morecausalmodels}.
%We ran the same experiments as we did for the law school data on the additional 
%datasets and found similar results.
%The figures for the additional experiments
%appear in Appendix \ref{sec:experiments}, as well as a link to our \href{https://anonymous.4open.science/r/simplifying_counterfactual_fairness-413B/}{\textbf{code}}, for reproducibility.
%
%Table \ref{tab:rmse} summarizes the error for each algorithm and
%example we consider.
%Of course, the full linear model (no fairness constraints)
%reliably achieves the lowest rMSE while Level 1 and Level 3 are close
%behind, since their predictions do not satisfy demographic parity.
%Level 2 tends to satisfy demographic parity but has higher error than
%Listing 1 and Listing 2.



%\subparagraph*{Experiments}
%Table \ref{tab:rmse} shows the rMSE for the six algorithms on
%all three data sets we explore: law school, default risk, and healthcare. As we discussed previously, we used the law school success data set from \cite{kusner2017counterfactual}.
%We sought a new real world data set that was not used in
%\cite{kusner2017counterfactual}:
%default risk is based on the Home Credit Default Risk data set \cite{kaggle}.
%We estimated a causal model based on observations of the default risk data, to mimic the ``domain expert'' process.
%We also sought to create a challenging synthetic data set that we could make match the causal model of a fake world almost exactly (because we could draw synthetic data directly from the fake structural model).
%Our synthetic data set on healthcare is very loosely based on \cite{obermeyer2019dissecting}. The synthetic scenario represents the ``ideal'' circumstance for counterfactual methods proposed by \cite{kusner2017counterfactual} where observations are
%drawn from the causal model.
%We include the figures for the structural causal models
%and prediction distributions in Appendix \ref{sec:experiments}.
%
%Our experiments with default risk demonstrated the difficulty in estimating a causal model (the ``domain expert'' process), and we noted that the ``levels'' proposed by \cite{kusner2017counterfactual} suffered from similar pitfalls to the law school example. For healthcare, because we had direct access to the ground truth causal model, Level 3 (which makes the strongest assumptions) performed well.
%However, direct access to a ground truth causal model is unrealistic. Across all the tests we conducted, our approaches (presented in Listings \ref{alg:normal} and \ref{alg:quantile}) consistently performed well while guaranteeing demographic parity and enforcing Assumption~\ref{req:preserve}.
% \vspace{-0.25cm}

%To derive the two simple algorithms for demographic parity,
%we used a strong assumption on the relative ranking of individuals
%made by a fair algorithm.
%Proposition \ref{prop:counterexample} shows that this assumption
%is not always true for counterfactually fair algorithms.
%We acknowledge that Assumption~\ref{req:preserve} may prevent us
%from producing the fairest model, from a causal perspective.
%However, we believe that preserved orderings are preferable to the
%highly unstable orderings in the levels of 
%\cite{kusner2017counterfactual}.
%One reason to prefer preserved orderings is that 
%even soft guarantees for relative orderings of within-group individuals 
%would lead to more transparent, trustworthy and ultimately 
%\textit{useful} counterfactually fair algorithms.
%Prior work already expands counterfactual fairness to deal with 
%between-group ranking \cite{yang2020causal}, and we hope that 
%our results encourage others to investigate counterfactually 
%fair models with theoretical guarantees.
%
%Under common distributional assumptions, we showed
%that counterfactual fairness implies demographic parity.
%This result offers a method for testing whether an
%algorithm is counterfactually fair.
%Furthermore, we derived two algorithms that satisfy demographic parity and
%preserve the ordering of outcomes within groups.
%Preserving the order of predictions within each
%group is a natural choice,
%we argue, when a causal model is unavailable.
%However, we show an example where a counterfactually fair
%algorithm induces a change in relative order.
%Our experiments on the three levels of counterfactual fairness proposed
%in \cite{kusner2017counterfactual} show that two of the
%three levels do not necessarily achieve demographic parity.
%Assuming the data is drawn from a distribution of latent variables
%that is independent of protected attributes, these findings
%suggest the two levels are not counterfactually fair.
%We further investigate the individual choices made by
%the levels and observe that individual predictions
%are highly unstable between different levels.
%We posit that even though preserving the order of predictions
%within groups is not always counterfactually fair,
%it is preferable to have a transparent and consistent
%policy over the apparent randomness in the three levels.
%
%We designed two algorithms to achieve demographic parity,
%which is a necessary condition for counterfactual fairness.
%% but they are not counterfactually fair.
%One important open question is how to design algorithms 
%with theoretical counterfactual fairness guarantees.

%In contrast, our two algorithms do preserve orderings
%in a principled manner while guaranteeing demographic parity.
%We believe that considering principled methods for automated 
%decision making procedures that account for protected
%attributes like race, gender, and age is vital for ethical
%implementations of machine learning,
%and leave open the problem of designing additional algorithms
%with counterfactual fairness guarantees.
